Extension of Dictionary-Based Compression Algorithms for the Quantitative Visualization of Patterns from Log Files

Many services today massively and continuously produce log files of different and varying formats. These logs are important since they contain information about the application activities, which is necessary for improvements by analyzing the behavior and maintaining the security and stability of the system. It is a common practice to store log files in a compressed form to reduce the sheer size of these files. A compression algorithm identifies frequent patterns in a log file to remove redundant information. This work presents an approach to detect frequent patterns in textual data that can be simultaneously registered during the file compression process with low consumption of resources. The log file can be visualized with the possibility to explore the extracted patterns using metrics based on such properties as frequency, length and root prefixes of the acquired pattern. This allows an analyst to gain the relevant insights more efficiently reducing the need for manual labor-intensive inspection in the log data. The extension of the implemented dictionary-based compression algorithm has the advantage of recognizing patterns in log files of any format and eliminates the need to manually perform preparation for any preprocessing of log files.

==> content/main.tex <==
% ---------------------------------------------------------------------
% EG author guidelines plus sample file for EG publication using LaTeX2e input
% D.Fellner, v2.03, Dec 14, 2018

\title{Extension of Dictionary-Based Compression Algorithms for the Quantitative Visualization of Patterns from Log Files}

% for anonymous conference submission please enter your SUBMISSION ID
% instead of the author's name (and leave the affiliation blank) !!
% for final version: please provide your *own* ORCID in the brackets following \orcid; see https://orcid.org/ for more details.
\author[I. Cherepanov]
{\parbox{\textwidth}{\centering 
I. Cherepanov$^{1}$\orcid{0000-0001-9109-090X}, 
J.G. Joewono$^{1}$,
A. Kuijper$^{1,2}$\orcid{0000-0002-6413-0061},
J. Kohlhammer$^{1,2}$\orcid{0000-0003-1706-8979} \\
        }
        \\
% For Computer Graphics Forum: Please use the abbreviation of your first name.
{\parbox{\textwidth}{\centering 
$^{1}$Fraunhofer IGD, Germany \quad  $^{2}$Technische Universität Darmstadt, Germany 
       }
}
}
% ------------------------------------------------------------------------

% if the Editors-in-Chief have given you the data, you may uncomment
% the following five lines and insert it here
%
% \volume{36}   % the volume in which the issue will be published;
% \issue{1}     % the issue number of the publication
% \pStartPage{1}      % set starting page


%-------------------------------------------------------------------------
\begin{document}

% uncomment for using teaser
% \teaser{
%  \includegraphics[width=\linewidth]{eg_new}
%  \centering
%   \caption{New EG Logo}
% \label{fig:teaser}
%}

\maketitle
%-------------------------------------------------------------------------
\begin{abstract}
Many services today massively and continuously produce log files of different and varying formats.
These logs are important since they contain information about the application activities, which is necessary for improvements by analyzing the behavior and maintaining the security and stability of the system.
It is a common practice to store log files in a compressed form to reduce the sheer size of these files. 
A compression algorithm identifies frequent patterns in a log file to remove redundant information.
This work presents an approach to detect frequent patterns in textual data that can be simultaneously registered during the file compression process with low consumption of resources. 
The log file can be visualized with the possibility to explore the extracted patterns using metrics based on such properties as frequency, length and root prefixes of the acquired pattern. 
This allows an analyst to gain the relevant insights more efficiently reducing the need for manual labor-intensive inspection in the log data.
The extension of the implemented dictionary-based compression algorithm has the advantage of recognizing patterns in log files of any format and eliminates the need to manually perform preparation for any preprocessing of log files.
%-------------------------------------------------------------------------
%  ACM CCS 1998
%  (see https://www.acm.org/publications/computing-classification-system/1998)
% \begin{classification} % according to https://www.acm.org/publications/computing-classification-system/1998
% \CCScat{Computer Graphics}{I.3.3}{Picture/Image Generation}{Line and curve generation}
% \end{classification}
%-------------------------------------------------------------------------
%  ACM CCS 2012
%   (see https://www.acm.org/publications/class-2012)
%The tool at \url{http://dl.acm.org/ccs.cfm} can be used to generate
% CCS codes.
%Example:
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003120.10003145.10003147.10010365</concept_id>
<concept_desc>Human-centered computing~Visual analytics</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10010405.10010497.10010504.10010505</concept_id>
<concept_desc>Applied computing~Document analysis</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10002951.10002952.10003219.10003215</concept_id>
<concept_desc>Information systems~Extraction, transformation and loading</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Applied computing~Document analysis}
\ccsdesc[500]{Human-centered computing~Visual analytics}
\ccsdesc[500]{Information systems~Extraction, transformation and loading}


\printccsdesc   
\end{abstract}  
%-------------------------------------------------------------------------


\section{Introduction}
\input{content/intro.tex}

\section{Related Work}
\input{content/related.tex}

\section{Approach}

In this section, we focus on our proposed extension of the LZW algorithm and describe the encoding part of it in more detail.
Then we introduce the metrics that we created based on the frequency, length, and root prefix, which allow the user to sort the data from the dictionary and also on which the quantitative coloring of the log files is performed.
Finally. we describe the visualization of the quantitative properties on the original log file.
We developed our approach as a web-based prototype, from which we generated and represented the results in form of snippets from an exemplary log file.

\input{content/approach.tex}

\section{Usage Scenario}
\input{content/case_study.tex}
%-------------------------------------------------------------------------
\section{Discussion and Future Work}
\input{content/conclusion_futurework.tex}
\section{Conclusion}
\input{content/conclusion}


%% if specified like this the section will be committed in review mode
\section*{Acknowledgement}
This research work has been funded by the German Ministry of Education and Research and the Hessian State Ministry for Higher Education, Research and the Arts within their joint support of the National Research Center for Applied Cybersecurity ATHENE.

%\clearpage
%-------------------------------------------------------------------------
% bibtex
\bibliographystyle{eg-alpha-doi}
\bibliography{egbibsample}

% biblatex with biber
% \printbibliography                


\end{document}

